Swarm parameter measurement in hydrogen, considering secondary photonic electron emission

Discharges in hydrogen at pressures above $1\,$kPa and a reduced electric field of $E/N=100-200\,$Td show a characteristic current oscillation in Pulsed Townsend experiments. This is explained by secondary emission of electrons from the photo-cathode: some hundreds of nano-seconds after the laser-pulse that released the initial $10^4-10^6$ primary electrons, secondary electrons are emitted from the cathode. Mechanisms discussed in literature are UV-emission from neutral molecules, emission by positive ions reaching the cathode, and back-scattering of excited neutrals. For a measurement up to $500\,$Td and pressures up to $2\,$kPa we model different sources, and agree with previous findings that the observed secondary emission is purely due to ultra-violet light below $200\,$Td: the simulation fits with the complicated form of the oscillating waveform. Obtained swarm parameters agree well with the literature. Our findings suggest a very high efficiency of the photo-cathode for UV light of energies above $8\,$eV.

==> experimental_setup.tex <==
In our Pulsed Townsend experiment electrons drift in a homogeneous electric field in between two Rogowski shaped electrodes. They are released from a photo-cathode, implanted in the middle of the electrode, with a UV laser pulse of $1.5\,$ns duration at $20\,$Hz. The displacement current is recorded at the anode with a transimpedance amplifier. Details about the experiment can be found in~\cite{pascal}. We fit the waveforms using a finite volume simulation on GPUs, which is described in~\cite{hosl2017measurement}.
